As-Continuous-As-Possible Extrusion Fabrication of Surface Models

We propose a novel computational framework for optimizing the toolpath continuity in fabricating surface models on an extrusion-based 3D printer. Toolpath continuity has been a critical issue for extrusion-based fabrications that affects both quality and efficiency. Transfer moves cause non-smoothor bumpy surfaces and get worse for materials with large inertia like clay. For surface models, the effects of continuity are even more severe, in terms of surface quality and model stability. In this paper, we introduce an original criterion "one-path-patch" (OPP), for representing a shell surface patch that can be traversed in one path considering fabrication constraints. We study the properties of an OPP and the merging operations for OPPs, and propose a bottom-up OPP merging procedure for decomposing the given shell surface into a minimal number of OPPs and generating the "as-continuous-as-possible" (ACAP) toolpath. Furthermore, we customize the path planning algorithm with a curved layer printing scheme, which reduces the staircase defect and improves the toolpath continuity via possibly connecting multiple segments. We evaluate the ACAP algorithm for both ceramic and thermoplastic materials, and results demonstrate that it improves the fabrication of surface models in both surface quality and efficiency.

==> mathprelim.tex <==
\section{Mathematical Preliminaries}


\subsection{AAA}


